The Social Divide of Social Distancing: Shelter-in-Place Behavior in Santiago during the Covid-19 Pandemic

Voluntary shelter-in-place directives and lockdowns are the main non-pharmaceutical interventions that governments around the globe have used to contain the Covid-19 pandemic. In this paper we study the impact of such interventions in the capital of a developing country, Santiago, Chile, that exhibits large socioeconomic inequality. A distinctive feature of our study is that we use granular geolocated mobile phone data to construct mobility measures that capture (1) shelter-in-place behavior, and (2) trips within the city to destinations with potentially different risk profiles. Using panel data linear regression models we first show that the impact of social distancing measures and lockdowns on mobility is highly heterogeneous and dependent on socioeconomic levels. More specifically, our estimates indicate that while zones of high socioeconomic levels can exhibit reductions in mobility of around 50\% to 90\% depending on the specific mobility metric used, these reductions are only 20\% to 50\% for lower-income communities. The large reductions in higher-income communities are significantly driven by voluntary shelter-in-place behavior. Second, also using panel data methods we show that our mobility measures are important predictors of infections: roughly, a 10\% increase in mobility correlates with a 5\% increase in the rate of infection. Our results suggest that mobility is an important factor explaining differences in infections rates between high and low incomes areas within the city. Further, they confirm the challenges of reducing mobility in lower-income communities, where people generate their income from their daily work. To be effective, shelter-in-place restrictions in municipalities of low socioeconomic levels may need to be complemented by other supporting measures that enable their inhabitants to increase compliance.

==> figs_tabs/LockdownOnMobility/AddLockOther/PanelModels_FracOut_FullInteraction_LockLocal_LockOther__NominalData_robusterror_v1.tex <==
%% Resultados analysis_mobility_v13_EL.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.007   &&   0.011   &   0.005   &   0.007   \\
                &  (0.006)  &&  (0.021)  &  (0.010)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.169*** && -0.413*** & -0.176*** & -0.107*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.297*** && -0.644*** & -0.314*** & -0.205*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.264*** && -0.608*** & -0.267*** & -0.196*** \\
                &  (0.006)  &&  (0.026)  &  (0.012)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.258*** && -0.601*** & -0.264*** & -0.187*** \\
                &  (0.005)  &&  (0.026)  &  (0.011)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.247*** && -0.546*** & -0.264*** & -0.174*** \\
                &  (0.005)  &&  (0.021)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.251*** && -0.571*** & -0.262*** & -0.179*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.215*** && -0.532*** & -0.217*** & -0.152*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.194*** && -0.527*** & -0.199*** & -0.132*** \\
                &  (0.005)  &&  (0.017)  &  (0.010)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.211*** && -0.548*** & -0.216*** & -0.163*** \\
                &  (0.006)  &&  (0.018)  &  (0.011)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.381*** && -0.772*** & -0.387*** & -0.290*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.322*** && -0.670*** & -0.330*** & -0.239*** \\
                &  (0.004)  &&  (0.018)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.360*** && -0.740*** & -0.353*** & -0.281*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.373*** && -0.758*** & -0.368*** & -0.292*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.347*** && -0.730*** & -0.347*** & -0.262*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.361*** && -0.744*** & -0.364*** & -0.274*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.328*** && -0.687*** & -0.337*** & -0.240*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$& -0.029*** && -0.053*** & -0.031*** & -0.026*** \\
                &  (0.004)  &&  (0.014)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$LockOther_{it}$& -0.153*** && -0.142*** & -0.158*** & -0.104*** \\
                &  (0.011)  &&  (0.037)  &  (0.024)  &  (0.022)  \\
                &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.624 && \multicolumn{3}{c}{0.682 } \\ 
Adjusted R$^{2}$ &  0.602 && \multicolumn{3}{c}{0.663 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/CorrectionDataLoss/PanelModels_FracOut_moda.home5_FullInteraction_CorrectedData_v1.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd
\begin{tabular}{@{\extracolsep{-0pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     & 0.018***  &&  0.034**  &  0.019**  &   0.014*  \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.180*** && -0.414*** & -0.196*** & -0.115*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.350*** && -0.683*** & -0.389*** & -0.243*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.389*** && -0.749*** & -0.420*** & -0.288*** \\
                &  (0.004)  &&  (0.015)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.331*** && -0.680*** & -0.346*** & -0.245*** \\
                &  (0.004)  &&  (0.015)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.319*** && -0.601*** & -0.336*** & -0.246*** \\
                &  (0.004)  &&  (0.014)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.298*** && -0.578*** & -0.312*** & -0.230*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.254*** && -0.538*** & -0.258*** & -0.193*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.238*** && -0.533*** & -0.244*** & -0.178*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.275*** && -0.565*** & -0.284*** & -0.228*** \\
                &  (0.004)  &&  (0.013)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.419*** && -0.767*** & -0.431*** & -0.333*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.417*** && -0.734*** & -0.431*** & -0.337*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.404*** && -0.732*** & -0.398*** & -0.336*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.416*** && -0.752*** & -0.411*** & -0.346*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.401*** && -0.732*** & -0.400*** & -0.330*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.401*** && -0.742*** & -0.403*** & -0.326*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.394*** && -0.685*** & -0.415*** & -0.313*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.102*** && -0.090*** & -0.105*** & -0.072*** \\
                &  (0.003)  &&  (0.010)  &  (0.005)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.632 && \multicolumn{3}{c}{0.670 } \\ 
Adjusted R$^{2}$ &  0.610 && \multicolumn{3}{c}{0.650 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/CorrectionDataLoss/PanelModels_FracOut_moda.home5_FullInteraction_CorrectedData_v1_robusterror.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd corrected data and robust error
\begin{tabular}{@{\extracolsep{-0pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     & 0.018***  &&   0.034   &   0.019*  &   0.014*  \\
                &  (0.005)  &&  (0.019)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.180*** && -0.414*** & -0.196*** & -0.115*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.350*** && -0.683*** & -0.389*** & -0.243*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.389*** && -0.749*** & -0.420*** & -0.288*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.331*** && -0.680*** & -0.346*** & -0.245*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.319*** && -0.601*** & -0.336*** & -0.246*** \\
                &  (0.004)  &&  (0.016)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.298*** && -0.578*** & -0.312*** & -0.230*** \\
                &  (0.004)  &&  (0.015)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.254*** && -0.538*** & -0.258*** & -0.193*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.238*** && -0.533*** & -0.244*** & -0.178*** \\
                &  (0.004)  &&  (0.014)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.275*** && -0.565*** & -0.284*** & -0.228*** \\
                &  (0.004)  &&  (0.014)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.419*** && -0.767*** & -0.431*** & -0.333*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.417*** && -0.734*** & -0.431*** & -0.337*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.404*** && -0.732*** & -0.398*** & -0.336*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.416*** && -0.752*** & -0.411*** & -0.346*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.401*** && -0.732*** & -0.400*** & -0.330*** \\
                &  (0.004)  &&  (0.015)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.401*** && -0.742*** & -0.403*** & -0.326*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.394*** && -0.685*** & -0.415*** & -0.313*** \\
                &  (0.005)  &&  (0.016)  &  (0.011)  &  (0.009)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.102*** && -0.090*** & -0.105*** & -0.072*** \\
                 &  (0.002)  &&  (0.007)  &  (0.004)  &  (0.005)  \\
                 &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.632 && \multicolumn{3}{c}{0.670 } \\ 
Adjusted R$^{2}$ &  0.610 && \multicolumn{3}{c}{0.650 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/CorrectionDataLoss/PanelModels_MobRisk_moda.home5_FullInteraction_CorrectedData_v1.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd
\begin{tabular}{@{\extracolsep{-0pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &  0.033*** && -0.098*** &  0.042**  & 0.055***  \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.572*** && -1.329*** & -0.526*** & -0.442*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -1.015*** && -2.285*** & -0.936*** & -0.798*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.222*** && -2.733*** & -1.158*** & -0.952*** \\
                &  (0.008)  &&  (0.030)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.150*** && -2.704*** & -1.085*** & -0.866*** \\
                &  (0.008)  &&  (0.030)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.105*** && -2.438*** & -1.076*** & -0.846*** \\
                &  (0.008)  &&  (0.027)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -1.009*** && -2.205*** & -1.006*** & -0.767*** \\
                &  (0.008)  &&  (0.026)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.895*** && -2.025*** & -0.894*** & -0.672*** \\
                &  (0.008)  &&  (0.026)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.896*** && -2.047*** & -0.904*** & -0.678*** \\
                &  (0.009)  &&  (0.026)  &  (0.015)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.979*** && -2.176*** & -1.005*** & -0.774*** \\
                &  (0.009)  &&  (0.026)  &  (0.016)  &  (0.015)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.277*** && -2.737*** & -1.246*** & -0.977*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.280*** && -2.764*** & -1.248*** & -0.975*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.252*** && -2.733*** & -1.188*** & -0.974*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.297*** && -2.807*** & -1.245*** & -1.003*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.274*** && -2.764*** & -1.221*** & -0.985*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.275*** && -2.765*** & -1.238*** & -0.973*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.254*** && -2.712*** & -1.218*** & -0.958*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.221*** && -0.307*** & -0.140*** & -0.170*** \\
                &  (0.006)  &&  (0.020)  &  (0.009)  &  (0.010)  \\
                &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          & 0.755  && \multicolumn{3}{c}{ 0.834} \\ 
Adjusted R$^{2}$ & 0.740  && \multicolumn{3}{c}{ 0.824} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/CorrectionDataLoss/PanelModels_MobRisk_moda.home5_FullInteraction_CorrectedData_v1_robusterror.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd
\begin{tabular}{@{\extracolsep{-0pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.033   &&  -0.098*  &   0.042   &  0.055*   \\
                &  (0.017)  &&  (0.042)  &  (0.027)  &  (0.023)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.572*** && -1.329*** & -0.526*** & -0.442*** \\
                &  (0.014)  &&  (0.035)  &  (0.022)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -1.015*** && -2.285*** & -0.936*** & -0.798*** \\
                &  (0.013)  &&  (0.033)  &  (0.021)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.222*** && -2.733*** & -1.158*** & -0.952*** \\
                &  (0.014)  &&  (0.038)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.150*** && -2.704*** & -1.085*** & -0.866*** \\
                &  (0.014)  &&  (0.039)  &  (0.023)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.105*** && -2.438*** & -1.076*** & -0.846*** \\
                &  (0.014)  &&  (0.035)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -1.009*** && -2.205*** & -1.006*** & -0.767*** \\
                &  (0.013)  &&  (0.033)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.895*** && -2.025*** & -0.894*** & -0.672*** \\
                &  (0.013)  &&  (0.033)  &  (0.022)  &  (0.017)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.896*** && -2.047*** & -0.904*** & -0.678*** \\
                &  (0.013)  &&  (0.032)  &  (0.021)  &  (0.017)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.979*** && -2.176*** & -1.005*** & -0.774*** \\
                &  (0.013)  &&  (0.033)  &  (0.021)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.277*** && -2.737*** & -1.246*** & -0.977*** \\
                &  (0.014)  &&  (0.034)  &  (0.021)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.280*** && -2.764*** & -1.248*** & -0.975*** \\
                &  (0.014)  &&  (0.034)  &  (0.021)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.252*** && -2.733*** & -1.188*** & -0.974*** \\
                &  (0.014)  &&  (0.033)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.297*** && -2.807*** & -1.245*** & -1.003*** \\
                &  (0.014)  &&  (0.033)  &  (0.021)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.274*** && -2.764*** & -1.221*** & -0.985*** \\
                &  (0.014)  &&  (0.033)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.275*** && -2.765*** & -1.238*** & -0.973*** \\
                &  (0.014)  &&  (0.034)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.254*** && -2.712*** & -1.218*** & -0.958*** \\
                &  (0.014)  &&  (0.033)  &  (0.023)  &  (0.019)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.221*** && -0.307*** & -0.140*** & -0.170*** \\
                &  (0.004)  &&  (0.015)  &  (0.007)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          & 0.755  && \multicolumn{3}{c}{ 0.834} \\ 
Adjusted R$^{2}$ & 0.740  && \multicolumn{3}{c}{ 0.824} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/InfectionsOnMobility/tab_Movilidad_lockdowns_contagios_week9-26.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd agregando nuevos sintomas
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{11}$     & -0.176*** && -0.424*** & -0.181*** & -0.115*** \\
                &  (0.003)  &&  (0.010)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.305*** && -0.656*** & -0.319*** & -0.213*** \\
                &  (0.003)  &&  (0.010)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.318*** && -0.703*** & -0.325*** & -0.230*** \\
                &  (0.003)  &&  (0.012)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.311*** && -0.694*** & -0.321*** & -0.219*** \\
                &  (0.003)  &&  (0.012)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.284*** && -0.607*** & -0.302*** & -0.199*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.280*** && -0.597*** & -0.290*** & -0.202*** \\
                &  (0.003)  &&  (0.010)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.250*** && -0.560*** & -0.249*** & -0.178*** \\
                &  (0.003)  &&  (0.010)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.250*** && -0.561*** & -0.246*** & -0.170*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.298*** && -0.592*** & -0.283*** & -0.222*** \\
                &  (0.004)  &&  (0.011)  &  (0.007)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.430*** && -0.788*** & -0.398*** & -0.308*** \\
                &  (0.004)  &&  (0.011)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.375*** && -0.686*** & -0.342*** & -0.257*** \\
                &  (0.005)  &&  (0.011)  &  (0.007)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.412*** && -0.756*** & -0.365*** & -0.300*** \\
                &  (0.005)  &&  (0.011)  &  (0.007)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.425*** && -0.774*** & -0.380*** & -0.311*** \\
                &  (0.005)  &&  (0.011)  &  (0.007)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.390*** && -0.745*** & -0.357*** & -0.279*** \\
                &  (0.004)  &&  (0.011)  &  (0.006)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.398*** && -0.758*** & -0.373*** & -0.289*** \\
                &  (0.004)  &&  (0.011)  &  (0.006)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.356*** && -0.700*** & -0.345*** & -0.254*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.092*** && -0.089*** & -0.082*** & -0.062*** \\
                &  (0.002)  &&  (0.008)  &  (0.004)  &  (0.004)  \\
                &           &&           &           &           \\[-1.1ex]
$Infections _{c(i),t-1}$ & 0.0001*** &&  0.00002* &           &           \\
                         & (0.00001) && (0.00001) &           &           \\
                         &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 27,673 && \multicolumn{3}{c}{27,673} \\ 
R$^{2}$          &  0.567 && \multicolumn{3}{c}{0.614 } \\ 
Adjusted R$^{2}$ &  0.540 && \multicolumn{3}{c}{0.589 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/InfectionsOnMobility/tab_Movilidad_lockdowns_contagios_week9-26_robust.tex <==
%% analysis_mobility_v16_EL_week9-26_Appendix.Rmd agregando nuevos sintomas
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{11}$     & -0.176*** && -0.424*** & -0.181*** & -0.115*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.305*** && -0.656*** & -0.319*** & -0.213*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.318*** && -0.703*** & -0.325*** & -0.230*** \\
                &  (0.004)  &&  (0.018)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.311*** && -0.694*** & -0.321*** & -0.219*** \\
                &  (0.004)  &&  (0.018)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.284*** && -0.607*** & -0.302*** & -0.199*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.280*** && -0.597*** & -0.290*** & -0.202*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.250*** && -0.560*** & -0.249*** & -0.178*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.250*** && -0.561*** & -0.246*** & -0.170*** \\
                &  (0.005)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.298*** && -0.592*** & -0.283*** & -0.222*** \\
                &  (0.005)  &&  (0.016)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.430*** && -0.788*** & -0.398*** & -0.308*** \\
                &  (0.006)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.375*** && -0.686*** & -0.342*** & -0.257*** \\
                &  (0.006)  &&  (0.018)  &  (0.009)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.412*** && -0.756*** & -0.365*** & -0.300*** \\
                &  (0.006)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.425*** && -0.774*** & -0.380*** & -0.311*** \\
                &  (0.006)  &&  (0.017)  &  (0.009)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.390*** && -0.745*** & -0.357*** & -0.279*** \\
                &  (0.006)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.398*** && -0.758*** & -0.373*** & -0.289*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.356*** && -0.700*** & -0.345*** & -0.254*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.092*** && -0.089*** & -0.082*** & -0.062*** \\
                 &  (0.002)  &&  (0.007)  &  (0.003)  &  (0.004)  \\
                 &           &&           &           &           \\[-1.1ex]
$Infections _{c(i),t-1}$ & 0.0001*** &&  0.00002* &           &           \\
                         & (0.00001) && (0.00001) &           &           \\
                         &           &&           &           &           \\[-2.1ex]

\hline \\[-1.8ex] 
Observations     & 27,673 && \multicolumn{3}{c}{27,673} \\ 
R$^{2}$          &  0.567 && \multicolumn{3}{c}{0.614 } \\ 
Adjusted R$^{2}$ &  0.540 && \multicolumn{3}{c}{0.589 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/InfectionsOnMobility/tab_Movilidad_lockdowns_contagios_week9-26_v2.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{$log(MobOut_{it})$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{it}$ & $-$0.092$^{***}$ &  \\ 
  & (0.002) &  \\ 
  & & \\ 
 $LockLocal_{it}$:$HighSeg_i$ &  & $-$0.089$^{***}$ \\ 
  &  & (0.007) \\ 
  & & \\ 
 $LockLocal_{it}$:$MedSeg_i$ &  & $-$0.082$^{***}$ \\ 
  &  & (0.003) \\ 
  & & \\ 
 $LockLocal_{it}$:$LowSeg_i$ &  & $-$0.062$^{***}$ \\ 
  &  & (0.004) \\ 
  & & \\ 
 $Infections_{c(i),t-1}$ & 0.0001$^{***}$ & 0.00002$^{*}$ \\ 
  & (0.00001) & (0.00001) \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 27,673 & 27,673 \\ 
R$^{2}$ & 0.567 & 0.614 \\ 
Adjusted R$^{2}$ & 0.540 & 0.589 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/PanelModels_FracOut_moda.home5_FullInteraction_NominalData_v4.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &  0.007*   &&   0.011   &   0.005   &   0.007   \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.169*** && -0.413*** & -0.176*** & -0.107*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.297*** && -0.644*** & -0.314*** & -0.205*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.311*** && -0.691*** & -0.320*** & -0.221*** \\
                &  (0.003)  &&  (0.013)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.304*** && -0.682*** & -0.316*** & -0.211*** \\
                &  (0.003)  &&  (0.013)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.276*** && -0.595*** & -0.297*** & -0.190*** \\
                &  (0.003)  &&  (0.012)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.270*** && -0.586*** & -0.284*** & -0.192*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.237*** && -0.548*** & -0.242*** & -0.169*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.227*** && -0.548*** & -0.238*** & -0.158*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.262*** && -0.578*** & -0.272*** & -0.206*** \\
                &  (0.004)  &&  (0.011)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.381*** && -0.772*** & -0.387*** & -0.290*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.322*** && -0.670*** & -0.330*** & -0.239*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.360*** && -0.740*** & -0.353*** & -0.281*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.373*** && -0.758*** & -0.368*** & -0.292*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.347*** && -0.730*** & -0.347*** & -0.262*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.361*** && -0.744*** & -0.364*** & -0.274*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.327*** && -0.687*** & -0.336*** & -0.240*** \\
                &  (0.003)  &&  (0.011)  &  (0.006)  &  (0.005)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.086*** && -0.089*** & -0.084*** & -0.060*** \\
                &  (0.002)  &&  (0.009)  &  (0.004)  &  (0.004)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,216 && \multicolumn{3}{c}{29,216} \\ 
R$^{2}$          &  0.620 && \multicolumn{3}{c}{0.680 } \\ 
Adjusted R$^{2}$ &  0.597 && \multicolumn{3}{c}{0.661 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/PanelModels_FracOut_moda.home5_FullInteraction_NominalData_v4_robusterror.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.007   &&   0.011   &   0.005   &   0.007   \\
                &  (0.006)  &&  (0.021)  &  (0.010)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.169*** && -0.413*** & -0.176*** & -0.107*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.297*** && -0.644*** & -0.314*** & -0.205*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.311*** && -0.691*** & -0.320*** & -0.221*** \\
                &  (0.004)  &&  (0.019)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.304*** && -0.682*** & -0.316*** & -0.211*** \\
                &  (0.004)  &&  (0.018)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.276*** && -0.595*** & -0.297*** & -0.190*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.270*** && -0.586*** & -0.284*** & -0.192*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.237*** && -0.548*** & -0.242*** & -0.169*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.227*** && -0.548*** & -0.238*** & -0.158*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.262*** && -0.578*** & -0.272*** & -0.207*** \\
                &  (0.004)  &&  (0.016)  &  (0.008)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.381*** && -0.772*** & -0.387*** & -0.290*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.322*** && -0.670*** & -0.330*** & -0.239*** \\
                &  (0.004)  &&  (0.018)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.360*** && -0.740*** & -0.353*** & -0.281*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.373*** && -0.758*** & -0.368*** & -0.292*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.347*** && -0.730*** & -0.347*** & -0.262*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.361*** && -0.744*** & -0.364*** & -0.274*** \\
                &  (0.004)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.328*** && -0.687*** & -0.337*** & -0.240*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.086*** && -0.089*** & -0.084*** & -0.060*** \\
                &  (0.002)  &&  (0.008)  &  (0.003)  &  (0.004)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.620 && \multicolumn{3}{c}{0.680 } \\ 
Adjusted R$^{2}$ &  0.598 && \multicolumn{3}{c}{0.661 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/PanelModels_MobRisk_moda.home5_FullInteraction_NominalData_v4.tex <==
%% Resultados analysis_mobility_v16_EL_week9-26.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.005   && -0.141*** &   0.011   &  0.032**  \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.552*** && -1.321*** & -0.497*** & -0.426*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.910*** && -2.196*** & -0.804*** & -0.709*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.069*** && -2.603*** & -0.979*** & -0.813*** \\
                &  (0.009)  &&  (0.029)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.092*** && -2.684*** & -1.027*** & -0.799*** \\
                &  (0.009)  &&  (0.029)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.018*** && -2.398*** & -0.995*** & -0.742*** \\
                &  (0.008)  &&  (0.027)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.953*** && -2.196*** & -0.952*** & -0.699*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.862*** && -2.027*** & -0.863*** & -0.629*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.875*** && -2.059*** & -0.888*** & -0.645*** \\
                &  (0.009)  &&  (0.026)  &  (0.015)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.946*** && -2.177*** & -0.974*** & -0.730*** \\
                &  (0.009)  &&  (0.026)  &  (0.015)  &  (0.014)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.202*** && -2.719*** & -1.163*** & -0.895*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.091*** && -2.614*** & -1.050*** & -0.782*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.162*** && -2.708*** & -1.095*** & -0.871*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.211*** && -2.783*** & -1.158*** & -0.903*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.163*** && -2.721*** & -1.110*** & -0.857*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.195*** && -2.740*** & -1.158*** & -0.879*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.124*** && -2.669*** & -1.074*** & -0.819*** \\
                &  (0.008)  &&  (0.026)  &  (0.014)  &  (0.012)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.201*** && -0.303*** & -0.112*** & -0.155*** \\
                &  (0.006)  &&  (0.020)  &  (0.009)  &  (0.010)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.715 && \multicolumn{3}{c}{0.814 } \\ 
Adjusted R$^{2}$ &  0.698 && \multicolumn{3}{c}{0.802 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/PanelModels_MobRisk_moda.home5_FullInteraction_NominalData_v4_robusterror.tex <==
%% Resultados analysis_mobility_v16_EL_week9-26.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.005   &&  -0.141** &   0.011   &   0.032   \\
                &  (0.018)  &&  (0.045)  &  (0.029)  &  (0.023)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.552*** && -1.321*** & -0.497*** & -0.426*** \\
                &  (0.015)  &&  (0.037)  &  (0.024)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.910*** && -2.196*** & -0.804*** & -0.709*** \\
                &  (0.014)  &&  (0.035)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.069*** && -2.603*** & -0.979*** & -0.813*** \\
                &  (0.014)  &&  (0.040)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.092*** && -2.684*** & -1.027*** & -0.799*** \\
                &  (0.014)  &&  (0.041)  &  (0.024)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.018*** && -2.398*** & -0.995*** & -0.742*** \\
                &  (0.014)  &&  (0.037)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.953*** && -2.196*** & -0.952*** & -0.699*** \\
                &  (0.014)  &&  (0.035)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.862*** && -2.027*** & -0.863*** & -0.629*** \\
                &  (0.014)  &&  (0.035)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.875*** && -2.059*** & -0.888*** & -0.645*** \\
                &  (0.014)  &&  (0.034)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.946*** && -2.177*** & -0.974*** & -0.730*** \\
                &  (0.014)  &&  (0.035)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.202*** && -2.719*** & -1.163*** & -0.895*** \\
                &  (0.014)  &&  (0.036)  &  (0.022)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.091*** && -2.614*** & -1.050*** & -0.782*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.162*** && -2.708*** & -1.095*** & -0.871*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.211*** && -2.783*** & -1.158*** & -0.903*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.163*** && -2.721*** & -1.110*** & -0.857*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.195*** && -2.740*** & -1.158*** & -0.879*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.124*** && -2.669*** & -1.074*** & -0.819*** \\
                &  (0.014)  &&  (0.036)  &  (0.023)  &  (0.018)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.201*** && -0.303*** & -0.112*** & -0.155*** \\
                &  (0.004)  &&  (0.016)  &  (0.007)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.715 && \multicolumn{3}{c}{0.814 } \\ 
Adjusted R$^{2}$ &  0.698 && \multicolumn{3}{c}{0.802 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/SumT1T2/PanelModels_FracOut_moda.home5_FullInteraction_NominalData_sumT1T2_v1.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26_sumT1T2.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &  0.007*   &&   0.014   &   0.005   &   0.007   \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.185*** && -0.450*** & -0.195*** & -0.118*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.323*** && -0.696*** & -0.344*** & -0.222*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.335*** && -0.740*** & -0.347*** & -0.238*** \\
                &  (0.004)  &&  (0.014)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.335*** && -0.741*** & -0.350*** & -0.234*** \\
                &  (0.004)  &&  (0.014)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.300*** && -0.639*** & -0.321*** & -0.209*** \\
                &  (0.004)  &&  (0.013)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.294*** && -0.630*** & -0.310*** & -0.209*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.264*** && -0.601*** & -0.273*** & -0.188*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.251*** && -0.596*** & -0.263*** & -0.174*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.287*** && -0.627*** & -0.298*** & -0.224*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.415*** && -0.829*** & -0.422*** & -0.316*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.346*** && -0.717*** & -0.357*** & -0.255*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.386*** && -0.788*** & -0.382*** & -0.300*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.401*** && -0.811*** & -0.399*** & -0.313*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.372*** && -0.780*** & -0.377*** & -0.278*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.387*** && -0.794*** & -0.394*** & -0.291*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.358*** && -0.744*** & -0.369*** & -0.262*** \\
                &  (0.004)  &&  (0.012)  &  (0.007)  &  (0.006)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.090*** && -0.089*** & -0.088*** & -0.064*** \\
                &  (0.002)  &&  (0.010)  &  (0.004)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.604 && \multicolumn{3}{c}{0.662 } \\ 
Adjusted R$^{2}$ &  0.581 && \multicolumn{3}{c}{0.641 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/SumT1T2/PanelModels_FracOut_moda.home5_FullInteraction_NominalData_sumT1T2_v1_robusterror.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26_sumT1T2.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobOut_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.007   &&   0.014   &   0.005   &   0.007   \\
                &  (0.006)  &&  (0.023)  &  (0.011)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.185*** && -0.450*** & -0.195*** & -0.118*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.323*** && -0.696*** & -0.344*** & -0.222*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -0.335*** && -0.740*** & -0.347*** & -0.238*** \\
                &  (0.005)  &&  (0.020)  &  (0.009)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -0.335*** && -0.741*** & -0.350*** & -0.234*** \\
                &  (0.005)  &&  (0.020)  &  (0.009)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -0.300*** && -0.639*** & -0.321*** & -0.209*** \\
                &  (0.005)  &&  (0.019)  &  (0.009)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -0.294*** && -0.630*** & -0.310*** & -0.209*** \\
                &  (0.005)  &&  (0.017)  &  (0.008)  &  (0.006)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.264*** && -0.601*** & -0.273*** & -0.188*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.251*** && -0.596*** & -0.263*** & -0.174*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -0.287*** && -0.627*** & -0.298*** & -0.224*** \\
                &  (0.005)  &&  (0.017)  &  (0.009)  &  (0.008)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -0.415*** && -0.829*** & -0.422*** & -0.316*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -0.346*** && -0.717*** & -0.357*** & -0.255*** \\
                &  (0.005)  &&  (0.019)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -0.386*** && -0.788*** & -0.382*** & -0.300*** \\
                &  (0.005)  &&  (0.019)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -0.401*** && -0.811*** & -0.399*** & -0.313*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -0.372*** && -0.780*** & -0.377*** & -0.278*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -0.387*** && -0.794*** & -0.394*** & -0.291*** \\
                &  (0.005)  &&  (0.018)  &  (0.009)  &  (0.007)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -0.358*** && -0.744*** & -0.369*** & -0.262*** \\
                &  (0.005)  &&  (0.018)  &  (0.010)  &  (0.008)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.090*** && -0.089*** & -0.088*** & -0.064*** \\
                &  (0.002)  &&  (0.008)  &  (0.004)  &  (0.005)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          &  0.604 && \multicolumn{3}{c}{0.662 } \\ 
Adjusted R$^{2}$ &  0.581 && \multicolumn{3}{c}{0.641 } \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/SumT1T2/PanelModels_MobRisk_moda.home5_FullInteraction_NominalData_sumT1T2_v1.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26_sumT1T2.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.004   && -0.148*** &   0.010   &  0.033*   \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.599*** && -1.436*** & -0.542*** & -0.458*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.979*** && -2.385*** & -0.869*** & -0.756*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.131*** && -2.792*** & -1.044*** & -0.844*** \\
                &  (0.009)  &&  (0.032)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.171*** && -2.907*** & -1.109*** & -0.841*** \\
                &  (0.009)  &&  (0.032)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.083*** && -2.598*** & -1.067*** & -0.771*** \\
                &  (0.009)  &&  (0.030)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -1.018*** && -2.388*** & -1.026*** & -0.728*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.934*** && -2.227*** & -0.945*** & -0.664*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.939*** && -2.242*** & -0.962*** & -0.674*** \\
                &  (0.010)  &&  (0.028)  &  (0.016)  &  (0.014)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -1.013*** && -2.370*** & -1.053*** & -0.764*** \\
                &  (0.010)  &&  (0.028)  &  (0.017)  &  (0.016)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.284*** && -2.948*** & -1.253*** & -0.937*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.158*** && -2.834*** & -1.129*** & -0.805*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.234*** && -2.925*** & -1.176*** & -0.902*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.287*** && -3.013*** & -1.244*** & -0.935*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.234*** && -2.943*** & -1.193*** & -0.883*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.267*** && -2.959*** & -1.242*** & -0.907*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.206*** && -2.908*** & -1.162*** & -0.858*** \\
                &  (0.009)  &&  (0.028)  &  (0.016)  &  (0.013)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.210*** && -0.327*** & -0.115*** & -0.162*** \\
                &  (0.006)  &&  (0.022)  &  (0.010)  &  (0.011)  \\
                &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          & 0.700  && \multicolumn{3}{c}{ 0.805} \\ 
Adjusted R$^{2}$ & 0.682  && \multicolumn{3}{c}{ 0.793} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/SumT1T2/PanelModels_MobRisk_moda.home5_FullInteraction_NominalData_sumT1T2_v1_robusterror.tex <==
%% Resultados analysis_mobility_v15_EL_week9-26_sumT1T2.Rmd
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log(MobRisk_{it})$}\\ 
\\[-1.8ex] & (1) && \multicolumn{3}{c}{(2)} \\ 
\cline{2-2}\cline{4-6}
        &&& HighSEG & MedSEG & LowSEG  \\
% \cline{2-2}\cline{4-6}
 \\[-1.8ex] 
$\tau_{10}$     &   0.004   && -0.148**  &   0.010   &   0.033   \\
                &  (0.020)  &&  (0.049)  &  (0.032)  &  (0.025)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{11}$     & -0.599*** && -1.436*** & -0.542*** & -0.458*** \\
                &  (0.016)  &&  (0.041)  &  (0.026)  &  (0.021)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{12}$     & -0.979*** && -2.385*** & -0.869*** & -0.756*** \\
                &  (0.015)  &&  (0.038)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{13}$     & -1.131*** && -2.792*** & -1.044*** & -0.844*** \\
                &  (0.015)  &&  (0.044)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{14}$     & -1.171*** && -2.907*** & -1.109*** & -0.841*** \\
                &  (0.016)  &&  (0.045)  &  (0.026)  &  (0.021)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{15}$     & -1.083*** && -2.598*** & -1.067*** & -0.771*** \\
                &  (0.015)  &&  (0.041)  &  (0.026)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{16}$     & -1.018*** && -2.388*** & -1.026*** & -0.728*** \\
                &  (0.015)  &&  (0.038)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{17}$     & -0.934*** && -2.227*** & -0.945*** & -0.664*** \\
                &  (0.015)  &&  (0.038)  &  (0.025)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{18}$     & -0.939*** && -2.242*** & -0.962*** & -0.674*** \\
                &  (0.015)  &&  (0.038)  &  (0.025)  &  (0.019)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{19}$     & -1.013*** && -2.370*** & -1.053*** & -0.764*** \\
                &  (0.015)  &&  (0.038)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{20}$     & -1.284*** && -2.948*** & -1.253*** & -0.937*** \\
                &  (0.015)  &&  (0.040)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{21}$     & -1.158*** && -2.834*** & -1.129*** & -0.805*** \\
                &  (0.015)  &&  (0.040)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{22}$     & -1.234*** && -2.925*** & -1.176*** & -0.902*** \\
                &  (0.015)  &&  (0.039)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{23}$     & -1.287*** && -3.013*** & -1.244*** & -0.935*** \\
                &  (0.015)  &&  (0.039)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{24}$     & -1.234*** && -2.943*** & -1.193*** & -0.883*** \\
                &  (0.016)  &&  (0.039)  &  (0.026)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{25}$     & -1.267*** && -2.959*** & -1.242*** & -0.907*** \\
                &  (0.016)  &&  (0.039)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-2.1ex]
$\tau_{26}$     & -1.206*** && -2.908*** & -1.162*** & -0.858*** \\
                &  (0.015)  &&  (0.039)  &  (0.025)  &  (0.020)  \\
                &           &&           &           &           \\[-1.ex]
$LockLocal_{it}$ & -0.210*** && -0.327*** & -0.115*** & -0.162*** \\
                 &  (0.005)  &&  (0.017)  &  (0.008)  &  (0.008)  \\
                 &           &&           &           &           \\[-2.1ex]
\hline \\[-1.8ex] 
Observations     & 29,214 && \multicolumn{3}{c}{29,214} \\ 
R$^{2}$          & 0.700  && \multicolumn{3}{c}{ 0.805} \\ 
Adjusted R$^{2}$ & 0.682  && \multicolumn{3}{c}{ 0.793} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/SummaryStatistics.tex <==

\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
$MobOut_{it}$ & 0.01 & 0.01 & 0.001 & 0.01 & 0.10 \\ 
$MobRisk_{it}$ & 0.55 & 0.14 & 0.12 & 0.54 & 1.00 \\ 
$LockLocal_{i}$ & 0.12 & 0.33 & 0.00 & 0.00 & 1.00 \\ 
$LockOther_{i}$ & 0.14 & 0.22 & 0.00 & 0.00 & 1.00 \\ 
$HighSEG_i$ & 0.11 & 0.25 & 0.00 & 0.00 & 1.00 \\ 
$MedSEG_i$ & 0.40 & 0.33 & 0.00 & 0.34 & 1.00 \\ 
$LowSEG_i$ & 0.48 & 0.37 & 0.00 & 0.49 & 1.00 \\ 
$Infections_{c(i),t-1}$ & 206.48 & 208.03 & 0.00 & 146.54 & 1,389.61 \\ 
\hline \\[-1.8ex] 
\end{tabular} 

==> figs_tabs/LockdownOnMobility/summary_stats_all.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-.8ex] 
\multicolumn{6}{l}{Census zone level}\\\cline{1-1}
$MobOut_{it}$ & 0.55 & 0.14 & 0.12 & 0.54 & 1.00 \\ 
$MobRisk_{it}$ & 1.19 & 0.77 & 0.14 & 0.97 & 10.26 \\ 
$LockLocal_{i}$ & 0.12 & 0.33 & 0.00 & 0.00 & 1.00 \\ 
$LockOther_{i}$ & 0.14 & 0.22 & 0.00 & 0.00 & 1.00 \\ 
$HighSEG_i$ & 0.11 & 0.25 & 0.00 & 0.00 & 1.00 \\ 
$MedSEG_i$ & 0.40 & 0.33 & 0.00 & 0.34 & 1.00 \\ 
$LowSEG_i$ & 0.48 & 0.37 & 0.00 & 0.49 & 1.00 \\ 
$Infections_{c(i),t-1}$ & 206.48 & 208.03 & 0.00 & 146.54 & 1,389.61 \\ \\[-.8ex]
\multicolumn{6}{l}{Municipality level}\\\cline{1-1}
$MobOut_{k,t-1}$ & 0.53 & 0.06 & 0.33 & 0.54 & 0.72 \\ 
$MobRisk_{k,t-1}$ & 0.89 & 0.45 & 0.24 & 0.79 & 5.39 \\ 
$LockLocal_{k,t-1}$ & 0.16 & 0.33 & 0.00 & 0.00 & 1.00 \\ 
$R_{kt}$ & 1.30 & 0.68 & 0.56 & 1.05 & 4.00 \\ 
\hline \\[-1.8ex] 
\end{tabular} 




==> figs_tabs/mobility_Rt/Rt_lag.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{R} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 lag.frac.lock &  &  &  &  & $-$0.311$^{***}$ & $-$0.244$^{***}$ \\ 
  &  &  &  &  & (0.109) & (0.086) \\ 
  & & & & & & \\ 
 lag.mob.out.max & 3.093$^{**}$ &  & 0.012 &  & 0.024 &  \\ 
  & (1.205) &  & (0.913) &  & (1.605) &  \\ 
  & & & & & & \\ 
 lag.mob.risk.prop &  & 0.521$^{***}$ &  & 0.395$^{*}$ &  & 0.367$^{**}$ \\ 
  &  & (0.149) &  & (0.223) &  & (0.157) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.772 & 0.775 & 0.565 & 0.573 & 0.777 & 0.780 \\ 
Adjusted R$^{2}$ & 0.741 & 0.744 & 0.462 & 0.472 & 0.746 & 0.749 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_bip.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  & $-$0.132$^{**}$ \\ 
  &  & (0.052) \\ 
  & & \\ 
 $NormOutBip_{k,t-1}$ & 2.052$^{***}$ & 1.398$^{***}$ \\ 
  & (0.463) & (0.527) \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 \\ 
R$^{2}$ & 0.834 & 0.837 \\ 
Adjusted R$^{2}$ & 0.812 & 0.814 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_bip_TripRisk.tex <==
% \begin{table}[H] \centering 
%   \caption{Estimation results of panel regressions of $\log R_{kt}$} 
%   \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{log(R)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  &  & $-$0.191$^{***}$ & $-$0.185$^{***}$ \\ 
  &  &  & (0.052) & (0.057) \\ 
  $TripOut_{k,t-1}$ & 0.037$^{**}$ &  & 0.006 &  \\ 
  & (0.016) &  & (0.018) &  \\ 
  $TripRisk_{k,t-1}$ &  & 0.021$^{***}$ &  & 0.004 \\ 
  &  & (0.007) &  & (0.009) \\ 
 \hline \\[-1.8ex] 
Observations & 411 & 411 & 411 & 411 \\ 
R$^{2}$ & 0.828 & 0.829 & 0.834 & 0.834 \\ 
Adjusted R$^{2}$ & 0.804 & 0.806 & 0.811 & 0.811 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
% \end{table} 

==> figs_tabs/mobility_Rt/logRt_lag.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.786$^{***}$ \\ 
  & (0.509) \\ 
  & \\ 
 $\tau_{11}$ & $-$0.102 \\ 
  & (0.087) \\ 
  & \\ 
 $\tau_{12}$ & $-$0.707$^{***}$ \\ 
  & (0.115) \\ 
  & \\ 
 $\tau_{13}$ & $-$0.541$^{***}$ \\ 
  & (0.151) \\ 
  & \\ 
 $\tau_{14}$ & $-$0.482$^{***}$ \\ 
  & (0.160) \\ 
  & \\ 
 $\tau_{15}$ & $-$0.425$^{***}$ \\ 
  & (0.157) \\ 
  & \\ 
 $\tau_{16}$ & $-$0.078 \\ 
  & (0.146) \\ 
  & \\ 
 $\tau_{17}$ & 0.149 \\ 
  & (0.147) \\ 
  & \\ 
 $\tau_{18}$ & $-$0.163 \\ 
  & (0.139) \\ 
  & \\ 
 $\tau_{19}$ & $-$0.549$^{***}$ \\ 
  & (0.141) \\ 
  & \\ 
 $\tau_{20}$ & $-$0.641$^{***}$ \\ 
  & (0.162) \\ 
  & \\ 
 $\tau_{21}$ & $-$0.643$^{***}$ \\ 
  & (0.177) \\ 
  & \\ 
 $\tau_{22}$ & $-$0.722$^{***}$ \\ 
  & (0.160) \\ 
  & \\ 
 $\tau_{23}$ & $-$0.893$^{***}$ \\ 
  & (0.171) \\ 
  & \\ 
 $\tau_{24}$ & $-$0.860$^{***}$ \\ 
  & (0.175) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 510 \\ 
R$^{2}$ & 0.624 \\ 
Adjusted R$^{2}$ & 0.585 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag1_2.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
%   \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{log(R)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  &  &  &  & $-$0.193$^{**}$ & 0.015 \\ 
  &  &  &  &  & (0.075) & (0.054) \\ 
  & & & & & & \\ 
 $LockLocal_{k,t-2}$ &  &  &  &  & $-$0.042 & $-$0.100$^{**}$ \\ 
  &  &  &  &  & (0.071) & (0.049) \\ 
  & & & & & & \\ 
 $MobOut_{k,t-1}$ & 2.386$^{***}$ &  & 0.136 &  & 0.488 &  \\ 
  & (0.728) &  & (1.042) &  & (0.945) &  \\ 
  & & & & & & \\ 
 $MobOut_{k,t-2}$ & $-$1.144$^{*}$ &  & $-$1.107 &  & $-$1.789$^{**}$ &  \\ 
  & (0.675) &  & (0.726) &  & (0.877) &  \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-1}$ &  & 0.983$^{***}$ &  & 0.895$^{***}$ &  & 0.965$^{***}$ \\ 
  &  & (0.091) &  & (0.235) &  & (0.100) \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-2}$ &  & $-$0.676$^{***}$ &  & $-$0.889$^{***}$ &  & $-$0.698$^{***}$ \\ 
  &  & (0.059) &  & (0.150) &  & (0.063) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.830 & 0.878 & 0.576 & 0.656 & 0.836 & 0.880 \\ 
Adjusted R$^{2}$ & 0.807 & 0.861 & 0.472 & 0.572 & 0.812 & 0.862 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag2.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{log(R)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-2}$ &  &  &  &  & $-$0.176$^{***}$ & $-$0.145$^{***}$ \\ 
  &  &  &  &  & (0.058) & (0.043) \\ 
  & & & & & & \\ 
 $MobOut_{k,t-2}$ & $-$0.371 &  & $-$1.092 &  & $-$2.065$^{**}$ &  \\ 
  & (0.641) &  & (0.714) &  & (0.847) &  \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-2}$ &  & $-$0.287$^{***}$ &  & $-$0.751$^{***}$ &  & $-$0.332$^{***}$ \\ 
  &  & (0.054) &  & (0.151) &  & (0.055) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.825 & 0.838 & 0.576 & 0.626 & 0.830 & 0.843 \\ 
Adjusted R$^{2}$ & 0.802 & 0.816 & 0.475 & 0.537 & 0.806 & 0.821 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_100.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects and Threshold 100} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 lag.wnorm.out.max & 1.238$^{**}$ \\ 
  & (0.622) \\ 
  & \\ 
 week12 & $-$0.913$^{***}$ \\ 
  & (0.222) \\ 
  & \\ 
 week13 & $-$0.597$^{**}$ \\ 
  & (0.250) \\ 
  & \\ 
 week14 & $-$0.461$^{*}$ \\ 
  & (0.257) \\ 
  & \\ 
 week15 & $-$0.332 \\ 
  & (0.260) \\ 
  & \\ 
 week16 & 0.008 \\ 
  & (0.240) \\ 
  & \\ 
 week17 & 0.231 \\ 
  & (0.241) \\ 
  & \\ 
 week18 & $-$0.066 \\ 
  & (0.238) \\ 
  & \\ 
 week19 & $-$0.458$^{*}$ \\ 
  & (0.237) \\ 
  & \\ 
 week20 & $-$0.593$^{**}$ \\ 
  & (0.256) \\ 
  & \\ 
 week21 & $-$0.588$^{**}$ \\ 
  & (0.282) \\ 
  & \\ 
 week22 & $-$0.679$^{***}$ \\ 
  & (0.250) \\ 
  & \\ 
 week23 & $-$0.850$^{***}$ \\ 
  & (0.268) \\ 
  & \\ 
 week24 & $-$0.828$^{***}$ \\ 
  & (0.272) \\ 
  & \\ 
 week25 & $-$0.972$^{***}$ \\ 
  & (0.270) \\ 
  & \\ 
 week26 & $-$0.887$^{***}$ \\ 
  & (0.267) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 446 \\ 
R$^{2}$ & 0.776 \\ 
Adjusted R$^{2}$ & 0.748 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_150.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.807$^{***}$ \\ 
  & (0.593) \\ 
   
 $\tau_{12}$ & $-$0.351 \\ 
  & (0.283) \\ 
   
 $\tau_{13}$ & $-$0.067 \\ 
  & (0.304) \\ 
   
 $\tau_{14}$ & 0.022 \\ 
  & (0.312) \\ 
   
 $\tau_{15}$ & 0.219 \\ 
  & (0.309) \\ 
   
 $\tau_{16}$ & 0.432 \\ 
  & (0.289) \\ 
   
 $\tau_{17}$ & 0.682$^{**}$ \\ 
  & (0.291) \\ 
   
 $\tau_{18}$ & 0.381 \\ 
  & (0.287) \\ 
   
 $\tau_{19}$ & $-$0.013 \\ 
  & (0.286) \\ 
   
 $\tau_{20}$ & $-$0.124 \\ 
  & (0.304) \\ 
   
 $\tau_{21}$ & $-$0.089 \\ 
  & (0.329) \\ 
   
 $\tau_{22}$ & $-$0.217 \\ 
  & (0.299) \\ 
   
 $\tau_{23}$ & $-$0.367 \\ 
  & (0.316) \\ 
   
 $\tau_{24}$ & $-$0.340 \\ 
  & (0.319) \\ 
   
 $\tau_{25}$ & $-$0.487 \\ 
  & (0.317) \\ 
   
 $\tau_{26}$ & $-$0.405 \\ 
  & (0.314) \\ 
   
\hline \\[-1.8ex] 
Observations & 412 \\ 
R$^{2}$ & 0.825 \\ 
Adjusted R$^{2}$ & 0.802 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}

==> figs_tabs/mobility_Rt/logRt_lag_200.tex <==
% \begin{table}[!htbp] \centering 
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects and Threshold 200} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 lag.wnorm.out.max & 2.559$^{***}$ \\ 
  & (0.580) \\ 
  & \\ 
 week12 & $-$0.377 \\ 
  & (0.273) \\ 
  & \\ 
 week13 & 0.234 \\ 
  & (0.293) \\ 
  & \\ 
 week14 & 0.229 \\ 
  & (0.296) \\ 
  & \\ 
 week15 & 0.623$^{**}$ \\ 
  & (0.300) \\ 
  & \\ 
 week16 & 0.642$^{**}$ \\ 
  & (0.278) \\ 
  & \\ 
 week17 & 0.977$^{***}$ \\ 
  & (0.277) \\ 
  & \\ 
 week18 & 0.659$^{**}$ \\ 
  & (0.274) \\ 
  & \\ 
 week19 & 0.263 \\ 
  & (0.273) \\ 
  & \\ 
 week20 & 0.183 \\ 
  & (0.291) \\ 
  & \\ 
 week21 & 0.259 \\ 
  & (0.315) \\ 
  & \\ 
 week22 & 0.081 \\ 
  & (0.286) \\ 
  & \\ 
 week23 & $-$0.040 \\ 
  & (0.302) \\ 
  & \\ 
 week24 & $-$0.008 \\ 
  & (0.306) \\ 
  & \\ 
 week25 & $-$0.158 \\ 
  & (0.304) \\ 
  & \\ 
 week26 & $-$0.081 \\ 
  & (0.301) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 393 \\ 
R$^{2}$ & 0.846 \\ 
Adjusted R$^{2}$ & 0.824 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_D.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 2.792$^{***}$ \\ 
  & (0.816) \\ 
  & \\ 
 $D_k\cdot NormOut_{k,t-1}$ & $-$1.190 \\ 
  & (0.754) \\ 
  & \\ 
 $\tau_{11}$ & $-$0.109 \\ 
  & (0.086) \\ 
  & \\ 
 $\tau_{12}$ & $-$0.592$^{***}$ \\ 
  & (0.135) \\ 
  & \\ 
 $\tau_{13}$ & $-$0.354$^{*}$ \\ 
  & (0.193) \\ 
  & \\ 
 $\tau_{14}$ & $-$0.279 \\ 
  & (0.205) \\ 
  & \\ 
 $\tau_{15}$ & $-$0.227 \\ 
  & (0.201) \\ 
  & \\ 
 $\tau_{16}$ & 0.104 \\ 
  & (0.185) \\ 
  & \\ 
 $\tau_{17}$ & 0.330$^{*}$ \\ 
  & (0.187) \\ 
  & \\ 
 $\tau_{18}$ & 0.005 \\ 
  & (0.176) \\ 
  & \\ 
 $\tau_{19}$ & $-$0.377$^{**}$ \\ 
  & (0.178) \\ 
  & \\ 
 $\tau_{20}$ & $-$0.423$^{**}$ \\ 
  & (0.213) \\ 
  & \\ 
 $\tau_{21}$ & $-$0.404$^{*}$ \\ 
  & (0.233) \\ 
  & \\ 
 $\tau_{22}$ & $-$0.515$^{**}$ \\ 
  & (0.207) \\ 
  & \\ 
 $\tau_{23}$ & $-$0.664$^{***}$ \\ 
  & (0.225) \\ 
  & \\ 
 $\tau_{24}$ & $-$0.622$^{***}$ \\ 
  & (0.231) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 510 \\ 
R$^{2}$ & 0.627 \\ 
Adjusted R$^{2}$ & 0.587 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_D_150.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.569$^{**}$ \\ 
  & (0.703) \\ 
  & \\ 
 $D_k\cdot NormOut_{k,t-1}$ & 0.083 \\ 
  & (1.135) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 344 \\ 
R$^{2}$ & 0.024 \\ 
Adjusted R$^{2}$ & $-$0.134 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_D_all.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 2.134$^{***}$ & 1.978$^{***}$ & 2.495$^{***}$ \\ 
  & (0.777) & (0.725) & (0.701) \\ 
  
  $D_k\cdot NormOut_{k,t-1}$ & $-$1.671$^{*}$ & $-$0.413 & 0.202 \\ 
  & (0.907) & (1.019) & (0.973) \\ 
   
 $\tau_{12}$ & $-$0.887$^{***}$ & $-$0.405 & $-$0.362 \\ 
  & (0.221) & (0.304) & (0.291) \\ 
   
 $\tau_{13}$ & $-$0.548$^{**}$ & $-$0.121 & 0.249 \\ 
  & (0.250) & (0.320) & (0.308) \\ 
   
 $\tau_{14}$ & $-$0.412 & $-$0.028 & 0.253 \\ 
  & (0.256) & (0.327) & (0.312) \\ 
   
 $\tau_{15}$ & $-$0.277 & 0.163 & 0.639$^{**}$ \\ 
  & (0.260) & (0.325) & (0.314) \\ 
   
 $\tau_{16}$ & 0.043 & 0.380 & 0.665$^{**}$ \\ 
  & (0.239) & (0.309) & (0.297) \\ 
   
 $\tau_{17}$ & 0.267 & 0.629$^{**}$ & 0.997$^{***}$ \\ 
  & (0.240) & (0.309) & (0.296) \\ 
   
 $\tau_{18}$ & $-$0.027 & 0.333 & 0.684$^{**}$ \\ 
  & (0.237) & (0.307) & (0.293) \\ 
   
 $\tau_{19}$ & $-$0.428$^{*}$ & $-$0.067 & 0.283 \\ 
  & (0.236) & (0.306) & (0.292) \\ 
   
 $\tau_{20}$ & $-$0.529$^{**}$ & $-$0.171 & 0.201 \\ 
  & (0.256) & (0.318) & (0.304) \\ 
   
 $\tau_{21}$ & $-$0.499$^{*}$ & $-$0.134 & 0.275 \\ 
  & (0.284) & (0.338) & (0.325) \\ 
   
 $\tau_{22}$ & $-$0.630$^{**}$ & $-$0.267 & 0.102 \\ 
  & (0.250) & (0.316) & (0.302) \\ 
   
 $\tau_{23}$ & $-$0.777$^{***}$ & $-$0.412 & $-$0.021 \\ 
  & (0.269) & (0.328) & (0.315) \\ 
   
 $\tau_{24}$ & $-$0.750$^{***}$ & $-$0.386 & 0.010 \\ 
  & (0.273) & (0.330) & (0.317) \\ 
   
 $\tau_{25}$ & $-$0.898$^{***}$ & $-$0.532 & $-$0.139 \\ 
  & (0.270) & (0.329) & (0.316) \\ 
   
 $\tau_{26}$ & $-$0.816$^{***}$ & $-$0.451 & $-$0.061 \\ 
  & (0.267) & (0.327) & (0.314) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.780 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.752 & 0.803 & 0.826 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_D_all_nodummies.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 2.134$^{***}$ & 1.978$^{***}$ & 2.495$^{***}$ \\ 
  & (0.777) & (0.725) & (0.701) \\ 
  
  $D_k\cdot NormOut_{k,t-1}$ & $-$1.671$^{*}$ & $-$0.413 & 0.202 \\ 
  & (0.907) & (1.019) & (0.973) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.780 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.752 & 0.803 & 0.826 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_all.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.264$^{**}$ & 1.807$^{***}$ & 2.578$^{***}$ \\ 
  & (0.620) & (0.589) & (0.576) \\ 
   
 $\tau_{12}$ & $-$0.911$^{***}$ & $-$0.358 & $-$0.384 \\ 
  & (0.221) & (0.281) & (0.271) \\ 
   
 $\tau_{13}$ & $-$0.593$^{**}$ & $-$0.079 & 0.228 \\ 
  & (0.249) & (0.302) & (0.291) \\ 
   
 $\tau_{14}$ & $-$0.457$^{*}$ & 0.015 & 0.232 \\ 
  & (0.256) & (0.310) & (0.294) \\ 
   
 $\tau_{15}$ & $-$0.328 & 0.205 & 0.619$^{**}$ \\ 
  & (0.259) & (0.307) & (0.297) \\ 
   
 $\tau_{16}$ & 0.012 & 0.425 & 0.643$^{**}$ \\ 
  & (0.239) & (0.287) & (0.276) \\ 
   
 $\tau_{17}$ & 0.233 & 0.674$^{**}$ & 0.975$^{***}$ \\ 
  & (0.240) & (0.289) & (0.275) \\ 
   
 $\tau_{18}$ & $-$0.059 & 0.378 & 0.662$^{**}$ \\ 
  & (0.237) & (0.286) & (0.272) \\ 
   
 $\tau_{19}$ & $-$0.456$^{*}$ & $-$0.021 & 0.261 \\ 
  & (0.236) & (0.285) & (0.271) \\ 
   
 $\tau_{20}$ & $-$0.589$^{**}$ & $-$0.132 & 0.182 \\ 
  & (0.255) & (0.302) & (0.288) \\ 
   
 $\tau_{21}$ & $-$0.586$^{**}$ & $-$0.099 & 0.257 \\ 
  & (0.281) & (0.326) & (0.313) \\ 
   
 $\tau_{22}$ & $-$0.675$^{***}$ & $-$0.224 & 0.081 \\ 
  & (0.249) & (0.297) & (0.283) \\ 
   
 $\tau_{23}$ & $-$0.846$^{***}$ & $-$0.374 & $-$0.040 \\ 
  & (0.267) & (0.314) & (0.300) \\ 
   
 $\tau_{24}$ & $-$0.824$^{***}$ & $-$0.348 & $-$0.009 \\ 
  & (0.271) & (0.317) & (0.303) \\ 
   
 $\tau_{25}$ & $-$0.967$^{***}$ & $-$0.494 & $-$0.158 \\ 
  & (0.268) & (0.315) & (0.301) \\ 
   
 $\tau_{26}$ & $-$0.882$^{***}$ & $-$0.412 & $-$0.081 \\ 
  & (0.266) & (0.312) & (0.299) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.778 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.750 & 0.804 & 0.827 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_all_nodummies.tex <==
%   \caption{Estimation results of panel regressions of $\log R_{kt}$} 
%   \label{} 
% \small
% \begin{tabular}{@{\extracolsep{5pt}}lccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
%  & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
% \cline{2-4} 
% \\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
% \\[-1.8ex] & (1) & (2) & (3)\\ 
% \hline \\[-1.8ex] 
%  $NormOut_{k,t-1}$ & 1.264$^{**}$ & 1.807$^{***}$ & 2.578$^{***}$ \\ 
%   & (0.620) & (0.589) & (0.576) \\ 
% \hline \\[-1.8ex] 
% Observations & 446 & 412 & 393 \\ 
% R$^{2}$ & 0.778 & 0.827 & 0.848 \\ 
% Adjusted R$^{2}$ & 0.750 & 0.804 & 0.827 \\ 
% \hline 
% \hline \\[-1.8ex] 
% \textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
% \end{tabular} 


  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
$NormOut_{k,t-1}$ & 1.218$^{**}$ & 1.603$^{***}$ & 2.208$^{***}$ \\ 
  & (0.560) & (0.532) & (0.522) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 443 & 411 & 392 \\ 
R$^{2}$ & 0.785 & 0.829 & 0.854 \\ 
Adjusted R$^{2}$ & 0.758 & 0.806 & 0.833 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_cor.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 lag.wnorm.out.max.cor & 2.058$^{***}$ \\ 
  & (0.525) \\ 
  & \\ 
 week11 & $-$0.128 \\ 
  & (0.087) \\ 
  & \\ 
 week12 & $-$0.649$^{***}$ \\ 
  & (0.119) \\ 
  & \\ 
 week13 & $-$0.407$^{**}$ \\ 
  & (0.170) \\ 
  & \\ 
 week14 & $-$0.302 \\ 
  & (0.187) \\ 
  & \\ 
 week15 & $-$0.309$^{*}$ \\ 
  & (0.170) \\ 
  & \\ 
 week16 & 0.056 \\ 
  & (0.164) \\ 
  & \\ 
 week17 & 0.257 \\ 
  & (0.160) \\ 
  & \\ 
 week18 & $-$0.074 \\ 
  & (0.149) \\ 
  & \\ 
 week19 & $-$0.466$^{***}$ \\ 
  & (0.148) \\ 
  & \\ 
 week20 & $-$0.536$^{***}$ \\ 
  & (0.173) \\ 
  & \\ 
 week21 & $-$0.515$^{***}$ \\ 
  & (0.192) \\ 
  & \\ 
 week22 & $-$0.520$^{***}$ \\ 
  & (0.192) \\ 
  & \\ 
 week23 & $-$0.757$^{***}$ \\ 
  & (0.189) \\ 
  & \\ 
 week24 & $-$0.723$^{***}$ \\ 
  & (0.192) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 510 \\ 
R$^{2}$ & 0.628 \\ 
Adjusted R$^{2}$ & 0.589 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_cor_150.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects with Corrected Mobility} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $\widetilde{NormOut}_{k,t-1}$ & 1.291$^{**}$ \\ 
  & (0.534) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 344 \\ 
R$^{2}$ & 0.019 \\ 
Adjusted R$^{2}$ & $-$0.136 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_cor_all.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.444$^{***}$ & 1.410$^{***}$ & 1.883$^{***}$ \\ 
  & (0.446) & (0.423) & (0.414) \\ 
   
 $\tau_{12}$ & $-$0.824$^{***}$ & $-$0.436$^{*}$ & $-$0.492$^{*}$ \\ 
  & (0.207) & (0.261) & (0.257) \\ 
   
 $\tau_{13}$ & $-$0.442$^{*}$ & $-$0.136 & 0.098 \\ 
  & (0.235) & (0.279) & (0.269) \\ 
   
 $\tau_{14}$ & $-$0.290 & $-$0.034 & 0.097 \\ 
  & (0.241) & (0.286) & (0.270) \\ 
   
 $\tau_{15}$ & $-$0.172 & 0.134 & 0.457$^{*}$ \\ 
  & (0.240) & (0.279) & (0.268) \\ 
   
 $\tau_{16}$ & 0.152 & 0.364 & 0.499$^{**}$ \\ 
  & (0.224) & (0.264) & (0.251) \\ 
   
 $\tau_{17}$ & 0.360 & 0.598$^{**}$ & 0.814$^{***}$ \\ 
  & (0.222) & (0.262) & (0.248) \\ 
   
 $\tau_{18}$ & 0.046 & 0.285 & 0.479$^{**}$ \\ 
  & (0.216) & (0.256) & (0.242) \\ 
   
 $\tau_{19}$ & $-$0.363$^{*}$ & $-$0.124 & 0.065 \\ 
  & (0.213) & (0.254) & (0.240) \\ 
   
 $\tau_{20}$ & $-$0.450$^{*}$ & $-$0.214 & 0.007 \\ 
  & (0.233) & (0.272) & (0.258) \\ 
   
 $\tau_{21}$ & $-$0.407 & $-$0.173 & 0.084 \\ 
  & (0.258) & (0.294) & (0.280) \\ 
   
 $\tau_{22}$ & $-$0.453$^{*}$ & $-$0.218 & 0.025 \\ 
  & (0.248) & (0.286) & (0.272) \\ 
   
 $\tau_{23}$ & $-$0.675$^{***}$ & $-$0.440 & $-$0.198 \\ 
  & (0.248) & (0.285) & (0.271) \\ 
   
 $\tau_{24}$ & $-$0.654$^{***}$ & $-$0.419 & $-$0.174 \\ 
  & (0.249) & (0.286) & (0.273) \\ 
   
 $\tau_{25}$ & $-$0.805$^{***}$ & $-$0.570$^{**}$ & $-$0.329 \\ 
  & (0.246) & (0.284) & (0.270) \\ 
   
 $\tau_{26}$ & $-$0.716$^{***}$ & $-$0.481$^{*}$ & $-$0.241 \\ 
  & (0.246) & (0.283) & (0.269) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.781 & 0.828 & 0.849 \\ 
Adjusted R$^{2}$ & 0.754 & 0.805 & 0.827 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_cor_all_nodummies.tex <==
% \begin{table}[!htbp] \centering 
  \caption{Estimation results of panel regressions of $\log R_{kt}$ due to data loss using infection rate threshold of 150.}
%   \label{} 
  
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{log(R)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  &  &  &  & $-$0.205$^{***}$ & $-$0.144$^{***}$ \\ 
  &  &  &  &  & (0.065) & (0.049) \\ 
  & & & & & & \\ 
 $MobOut_{k,t-1}$ & 1.877$^{***}$ &  & 0.562 &  & $-$0.116 &  \\ 
  & (0.636) &  & (0.965) &  & (0.889) &  \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-1}$ &  & 0.419$^{***}$ &  & 0.580$^{**}$ &  & 0.305$^{***}$ \\ 
  &  & (0.096) &  & (0.284) &  & (0.102) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.829 & 0.834 & 0.571 & 0.580 & 0.834 & 0.838 \\ 
Adjusted R$^{2}$ & 0.806 & 0.812 & 0.468 & 0.481 & 0.811 & 0.815 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
% \end{table} 


%   \caption{Estimation results of panel regressions of $\log R_{kt}$} 
%   \label{} 
% \small 
% \begin{tabular}{@{\extracolsep{5pt}}lccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
%  & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
% \cline{2-4} 
% \\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
% \\[-1.8ex] & (1) & (2) & (3)\\ 
% \hline \\[-1.8ex] 
%  $NormOut_{k,t-1}$ & 1.444$^{***}$ & 1.410$^{***}$ & 1.883$^{***}$ \\ 
%   & (0.446) & (0.423) & (0.414) \\ 
% \hline \\[-1.8ex] 
% Observations & 446 & 412 & 393 \\ 
% R$^{2}$ & 0.781 & 0.828 & 0.849 \\ 
% Adjusted R$^{2}$ & 0.754 & 0.805 & 0.827 \\ 
% \hline 
% \hline \\[-1.8ex] 
% \textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
% \end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_curr_150.tex <==
  \caption{Estimation results of Panel Regressions of log(R) with Two Way Effects} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $R_{k,t-1}$ & 1.437$^{**}$ \\ 
  & (0.690) \\ 
  & \\ 
 $R_{kt}$ & 1.986$^{***}$ \\ 
  & (0.737) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 276 \\ 
R$^{2}$ & 0.059 \\ 
Adjusted R$^{2}$ & $-$0.131 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_lock_all_nodummies.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
$NormOut_{k,t-1}$ & $-$1.078 & 0.099 & 0.480 \\ 
  & (0.729) & (0.714) & (0.677) \\ 
  & & & \\ 
$FracLock_{k,t-1}\cdot1(t-1<20)$ & $-$0.301$^{***}$ & $-$0.193$^{***}$ & $-$0.228$^{***}$ \\ 
  & (0.063) & (0.062) & (0.058) \\ 
\hline \\[-1.8ex] 
Observations & 443 & 411 & 392 \\ 
R$^{2}$ & 0.796 & 0.834 & 0.860 \\ 
Adjusted R$^{2}$ & 0.770 & 0.811 & 0.840 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_sum.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 lag.wnorm.out.sum & 1.768$^{***}$ \\ 
  & (0.489) \\ 
  & \\ 
 week11 & $-$0.104 \\ 
  & (0.086) \\ 
  & \\ 
 week12 & $-$0.684$^{***}$ \\ 
  & (0.117) \\ 
  & \\ 
 week13 & $-$0.518$^{***}$ \\ 
  & (0.154) \\ 
  & \\ 
 week14 & $-$0.459$^{***}$ \\ 
  & (0.162) \\ 
  & \\ 
 week15 & $-$0.393$^{**}$ \\ 
  & (0.161) \\ 
  & \\ 
 week16 & $-$0.052 \\ 
  & (0.149) \\ 
  & \\ 
 week17 & 0.171 \\ 
  & (0.150) \\ 
  & \\ 
 week18 & $-$0.133 \\ 
  & (0.144) \\ 
  & \\ 
 week19 & $-$0.521$^{***}$ \\ 
  & (0.144) \\ 
  & \\ 
 week20 & $-$0.613$^{***}$ \\ 
  & (0.165) \\ 
  & \\ 
 week21 & $-$0.613$^{***}$ \\ 
  & (0.180) \\ 
  & \\ 
 week22 & $-$0.700$^{***}$ \\ 
  & (0.162) \\ 
  & \\ 
 week23 & $-$0.871$^{***}$ \\ 
  & (0.173) \\ 
  & \\ 
 week24 & $-$0.835$^{***}$ \\ 
  & (0.178) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 510 \\ 
R$^{2}$ & 0.626 \\ 
Adjusted R$^{2}$ & 0.587 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_sum_150.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.490$^{**}$ \\ 
  & (0.578) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 344 \\ 
R$^{2}$ & 0.022 \\ 
Adjusted R$^{2}$ & $-$0.133 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_sum_all.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $NormOut_{k,t-1}$ & 1.222$^{**}$ & 1.645$^{***}$ & 2.333$^{***}$ \\ 
  & (0.589) & (0.560) & (0.549) \\ 
   
 $\tau_{12}$ & $-$0.886$^{***}$ & $-$0.356 & $-$0.381 \\ 
  & (0.227) & (0.286) & (0.277) \\ 
   
 $\tau_{13}$ & $-$0.564$^{**}$ & $-$0.077 & 0.225 \\ 
  & (0.257) & (0.309) & (0.298) \\ 
   
 $\tau_{14}$ & $-$0.430 & 0.011 & 0.221 \\ 
  & (0.263) & (0.316) & (0.301) \\ 
   
 $\tau_{15}$ & $-$0.299 & 0.206 & 0.612$^{**}$ \\ 
  & (0.268) & (0.315) & (0.306) \\ 
   
 $\tau_{16}$ & 0.037 & 0.424 & 0.636$^{**}$ \\ 
  & (0.246) & (0.294) & (0.283) \\ 
   
 $\tau_{17}$ & 0.260 & 0.674$^{**}$ & 0.969$^{***}$ \\ 
  & (0.248) & (0.295) & (0.282) \\ 
   
 $\tau_{18}$ & $-$0.028 & 0.384 & 0.665$^{**}$ \\ 
  & (0.246) & (0.294) & (0.281) \\ 
   
 $\tau_{19}$ & $-$0.428$^{*}$ & $-$0.017 & 0.261 \\ 
  & (0.244) & (0.292) & (0.279) \\ 
   
 $\tau_{20}$ & $-$0.559$^{**}$ & $-$0.129 & 0.179 \\ 
  & (0.263) & (0.310) & (0.297) \\ 
   
 $\tau_{21}$ & $-$0.558$^{*}$ & $-$0.106 & 0.240 \\ 
  & (0.289) & (0.333) & (0.321) \\ 
   
 $\tau_{22}$ & $-$0.647$^{**}$ & $-$0.224 & 0.075 \\ 
  & (0.257) & (0.304) & (0.291) \\ 
   
 $\tau_{23}$ & $-$0.817$^{***}$ & $-$0.377 & $-$0.051 \\ 
  & (0.275) & (0.321) & (0.308) \\ 
   
 $\tau_{24}$ & $-$0.795$^{***}$ & $-$0.351 & $-$0.020 \\ 
  & (0.279) & (0.324) & (0.312) \\ 
   
 $\tau_{25}$ & $-$0.939$^{***}$ & $-$0.498 & $-$0.170 \\ 
  & (0.276) & (0.322) & (0.309) \\ 
   
 $\tau_{26}$ & $-$0.853$^{***}$ & $-$0.414 & $-$0.091 \\ 
  & (0.274) & (0.320) & (0.307) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.778 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.751 & 0.804 & 0.826 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_sum_all_nodummies.tex <==
% \begin{table}[!htbp] \centering 
  \caption{Estimation results of panel regressions of $\log R_{kt}$ with sum of time block flows using infection rate threshold of 150.} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{log(R)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  &  &  &  & $-$0.208$^{***}$ & $-$0.156$^{***}$ \\ 
  &  &  &  &  & (0.060) & (0.048) \\ 
  & & & & & & \\ 
 $MobOut_{k,t-1}$ & 1.816$^{***}$ &  & $-$0.499 &  & $-$0.196 &  \\ 
  & (0.688) &  & (1.010) &  & (0.896) &  \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-1}$ &  & 0.350$^{***}$ &  & 0.516$^{**}$ &  & 0.257$^{***}$ \\ 
  &  & (0.086) &  & (0.247) &  & (0.090) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.828 & 0.833 & 0.570 & 0.581 & 0.834 & 0.838 \\ 
Adjusted R$^{2}$ & 0.805 & 0.810 & 0.468 & 0.481 & 0.811 & 0.815 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
% \end{table} 

%   \caption{Estimation results of panel regressions of $\log R_{kt}$} 
%   \label{} 
% \small 
% \begin{tabular}{@{\extracolsep{5pt}}lccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
%  & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
% \cline{2-4} 
% \\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
% \\[-1.8ex] & (1) & (2) & (3)\\ 
% \hline \\[-1.8ex] 
%  $NormOut_{k,t-1}$ & 1.222$^{**}$ & 1.645$^{***}$ & 2.333$^{***}$ \\ 
%   & (0.589) & (0.560) & (0.549) \\ 

   
% \hline \\[-1.8ex] 
% Observations & 446 & 412 & 393 \\ 
% R$^{2}$ & 0.778 & 0.827 & 0.848 \\ 
% Adjusted R$^{2}$ & 0.751 & 0.804 & 0.826 \\ 
% \hline 
% \hline \\[-1.8ex] 
% \textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
% \end{tabular} 

==> figs_tabs/mobility_Rt/logRt_lag_weightedmob_all_nodummies.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $WeightedMob_{k,t-1}$ & 30.398$^{***}$ & 46.717$^{***}$ & 79.119$^{***}$ \\ 
  & (11.456) & (11.497) & (11.448) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 443 & 411 & 392 \\ 
R$^{2}$ & 0.786 & 0.833 & 0.865 \\ 
Adjusted R$^{2}$ & 0.759 & 0.810 & 0.846 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_loglag.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & log(R) \\ 
\hline \\[-1.8ex] 
 log(lag.wnorm.out.max) & 1.047$^{***}$ \\ 
  & (0.341) \\ 
  & \\ 
 week11 & $-$0.098 \\ 
  & (0.087) \\ 
  & \\ 
 week12 & $-$0.799$^{***}$ \\ 
  & (0.103) \\ 
  & \\ 
 week13 & $-$0.680$^{***}$ \\ 
  & (0.130) \\ 
  & \\ 
 week14 & $-$0.622$^{***}$ \\ 
  & (0.139) \\ 
  & \\ 
 week15 & $-$0.561$^{***}$ \\ 
  & (0.136) \\ 
  & \\ 
 week16 & $-$0.208 \\ 
  & (0.126) \\ 
  & \\ 
 week17 & 0.014 \\ 
  & (0.127) \\ 
  & \\ 
 week18 & $-$0.289$^{**}$ \\ 
  & (0.121) \\ 
  & \\ 
 week19 & $-$0.675$^{***}$ \\ 
  & (0.122) \\ 
  & \\ 
 week20 & $-$0.790$^{***}$ \\ 
  & (0.139) \\ 
  & \\ 
 week21 & $-$0.798$^{***}$ \\ 
  & (0.153) \\ 
  & \\ 
 week22 & $-$0.866$^{***}$ \\ 
  & (0.138) \\ 
  & \\ 
 week23 & $-$1.047$^{***}$ \\ 
  & (0.148) \\ 
  & \\ 
 week24 & $-$1.015$^{***}$ \\ 
  & (0.151) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 510 \\ 
R$^{2}$ & 0.623 \\ 
Adjusted R$^{2}$ & 0.584 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_loglag_150.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $\log NormOut_{k,t-1}$ & 1.010$^{***}$ \\ 
  & (0.374) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 344 \\ 
R$^{2}$ & 0.024 \\ 
Adjusted R$^{2}$ & $-$0.131 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_loglag_all.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $\log NormOut_{k,t-1}$ & 0.657 & 1.123$^{***}$ & 1.688$^{***}$ \\ 
  & (0.412) & (0.392) & (0.383) \\ 
   
 $\tau_{12}$ & $-$1.019$^{***}$ & $-$0.472$^{*}$ & $-$0.523$^{**}$ \\ 
  & (0.204) & (0.266) & (0.256) \\ 
   
 $\tau_{13}$ & $-$0.730$^{***}$ & $-$0.221 & 0.065 \\ 
  & (0.225) & (0.279) & (0.268) \\ 
   
 $\tau_{14}$ & $-$0.598$^{**}$ & $-$0.129 & 0.069 \\ 
  & (0.231) & (0.286) & (0.270) \\ 
   
 $\tau_{15}$ & $-$0.474$^{**}$ & 0.059 & 0.453$^{*}$ \\ 
  & (0.233) & (0.283) & (0.272) \\ 
   
 $\tau_{16}$ & $-$0.118 & 0.292 & 0.490$^{*}$ \\ 
  & (0.217) & (0.266) & (0.254) \\ 
   
 $\tau_{17}$ & 0.102 & 0.538$^{**}$ & 0.821$^{***}$ \\ 
  & (0.217) & (0.267) & (0.253) \\ 
   
 $\tau_{18}$ & $-$0.187 & 0.245 & 0.510$^{**}$ \\ 
  & (0.215) & (0.264) & (0.250) \\ 
   
 $\tau_{19}$ & $-$0.583$^{***}$ & $-$0.153 & 0.110 \\ 
  & (0.214) & (0.263) & (0.250) \\ 
   
 $\tau_{20}$ & $-$0.735$^{***}$ & $-$0.281 & 0.010 \\ 
  & (0.228) & (0.276) & (0.263) \\ 
   
 $\tau_{21}$ & $-$0.750$^{***}$ & $-$0.261 & 0.074 \\ 
  & (0.250) & (0.297) & (0.284) \\ 
   
 $\tau_{22}$ & $-$0.815$^{***}$ & $-$0.367 & $-$0.082 \\ 
  & (0.224) & (0.273) & (0.259) \\ 
   
 $\tau_{23}$ & $-$1.000$^{***}$ & $-$0.529$^{*}$ & $-$0.216 \\ 
  & (0.239) & (0.286) & (0.273) \\ 
   
 $\tau_{24}$ & $-$0.981$^{***}$ & $-$0.505$^{*}$ & $-$0.187 \\ 
  & (0.241) & (0.289) & (0.275) \\ 
   
 $\tau_{25}$ & $-$1.122$^{***}$ & $-$0.649$^{**}$ & $-$0.334 \\ 
  & (0.240) & (0.288) & (0.274) \\ 
   
 $\tau_{26}$ & $-$1.035$^{***}$ & $-$0.566$^{**}$ & $-$0.255 \\ 
  & (0.237) & (0.285) & (0.272) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.777 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.749 & 0.803 & 0.827 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_loglag_all_nodummies.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 $\log NormOut_{k,t-1}$ & 0.657 & 1.123$^{***}$ & 1.688$^{***}$ \\ 
  & (0.412) & (0.392) & (0.383) \\ 
   
\hline \\[-1.8ex] 
Observations & 446 & 412 & 393 \\ 
R$^{2}$ & 0.777 & 0.827 & 0.848 \\ 
Adjusted R$^{2}$ & 0.749 & 0.803 & 0.827 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/logRt_loglag_logcurr_150.tex <==
  \caption{Estimation results of Panel Regressions of $\log R_{kt}$ with Two Way Effects} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & $\log R_{kt}$ \\ 
\hline \\[-1.8ex] 
 $\log NormOut_{k,t-1}$ & 0.915$^{**}$ \\ 
  & (0.445) \\ 
  & \\ 
 $\log NormOut_{kt}$ & 1.146$^{**}$ \\ 
  & (0.477) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 276 \\ 
R$^{2}$ & 0.053 \\ 
Adjusted R$^{2}$ & $-$0.137 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}

==> figs_tabs/mobility_Rt/rev_logRt_lag.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{$\log R_{kt}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5)\\ 
\hline \\[-1.8ex] 
 $FracLock_{k,t-1}$ & $-$0.199$^{***}$ &  & $-$0.209$^{***}$ &  & $-$0.153$^{***}$ \\ 
  & (0.046) &  & (0.058) &  & (0.048) \\ 
  & & & & & \\ 
 $MobOut_{k,t-1}$ &  & 1.585$^{**}$ & $-$0.216 &  &  \\ 
  &  & (0.658) & (0.817) &  &  \\ 
  & & & & & \\ 
 $MobRisk_{k,t-1}$ &  &  &  & 34.662$^{***}$ & 25.152$^{***}$ \\ 
  &  &  &  & (8.445) & (8.856) \\ 
  & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 411 & 411 & 411 \\ 
R$^{2}$ & 0.834 & 0.828 & 0.834 & 0.833 & 0.838 \\ 
Adjusted R$^{2}$ & 0.811 & 0.805 & 0.811 & 0.810 & 0.815 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/rev_logRt_lag_adj.tex <==
  \caption{Estimation results of panel regressions of $\log R_{kt}$ adjusting for under-reporting using infection rate threshold of 150.} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{log(R.adj)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $LockLocal_{k,t-1}$ &  &  &  &  & $-$0.227$^{***}$ & $-$0.160$^{***}$ \\ 
  &  &  &  &  & (0.061) & (0.048) \\ 
  & & & & & & \\ 
 $MobOut_{k,t-1}$ & 1.746$^{**}$ &  & $-$0.950 &  & $-$0.490 &  \\ 
  & (0.683) &  & (1.057) &  & (0.903) &  \\ 
  & & & & & & \\ 
 $MobRisk_{k,t-1}$ &  & 0.339$^{***}$ &  & 0.612$^{**}$ &  & 0.238$^{***}$ \\ 
  &  & (0.084) &  & (0.257) &  & (0.088) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 411 & 411 & 204 & 204 & 411 & 411 \\ 
R$^{2}$ & 0.826 & 0.830 & 0.617 & 0.628 & 0.832 & 0.835 \\ 
Adjusted R$^{2}$ & 0.802 & 0.807 & 0.526 & 0.540 & 0.809 & 0.812 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> figs_tabs/mobility_Rt/summary_stats.tex <==
% \begin{table}[!htbp] \centering 
%   \caption{} 
%   \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
$MobOut_{k,t-1}$ & 411 & 0.529 & 0.064 & 0.326 & 0.508 & 0.572 & 0.721 \\ 
$MobRisk_{k,t-1}$ & 411 & 0.893 & 0.444 & 0.240 & 0.648 & 1.004 & 5.381 \\ 
$LockLocal_{k,t-1}$ & 411 & 0.164 & 0.330 & 0 & 0 & 0 & 1 \\ 
$R_{kt}$ & 411 & 1.297 & 0.678 & 0.559 & 0.822 & 1.549 & 4.000 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
% \end{table} 

% \begin{tabular}{@{\extracolsep{5pt}}lccccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
% Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ 
% \hline \\[-1.8ex] 
% $R_{kt}$ & 578 & 1.607 & 1.359 & 0.375 & 14.500 \\ 
% $NormOut_{k,t-1}$ & 578 & 0.773 & 0.116 & 0.483 & 1.025 \\ 
% \hline \\[-1.8ex] 
% \end{tabular} 

% \begin{tabular}{@{\extracolsep{-7pt}}lccccccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
% Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
% \hline \\[-1.8ex] 
% $R_{kt}$ & 344 & 1.400 & 0.678 & 0.428 & 0.906 & 1.768 & 4.308 \\ 
% $NormOut_{k,t-1}$ & 344 & 0.737 & 0.085 & 0.483 & 0.705 & 0.795 & 1.001 \\ 
% \hline \\[-1.8ex] 
% \end{tabular} 



% \begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
% Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
% \hline \\[-1.8ex] 
% logR & 344 & 0.239 & 0.427 & $-$0.848 & $-$0.099 & 0.570 & 1.460 \\ 
% lag.wnorm.out.max & 344 & 0.737 & 0.085 & 0.483 & 0.705 & 0.795 & 1.001 \\ 
% \hline \\[-1.8ex] 
% \end{tabular} 

==> figs_tabs/summary_demographics.tex <==

% Date and time: Wed, May 27, 2020 - 04:19:16
% \begin{table}[!htbp] \centering 
%   \caption{} 
%   \label{} 
\begin{tabular}{@{\extracolsep{-5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
Population & 3,708.157 & 1,274.876 & 10 & 3,661 & 11,031 \\ 
Fraction of male & 0.482 & 0.031 & 0.000 & 0.484 & 0.914 \\ 
Fraction above 65 & 0.111 & 0.052 & 0.000 & 0.117 & 0.291 \\ 
People per household & 3.054 & 0.694 & 1.000 & 3.210 & 15.236 \\ 
Fraction of inmigrants & 0.074 & 0.090 & 0.000 & 0.041 & 0.599 \\ 
Households density & 56.757 & 72.220 & 0.021 & 42.100 & 952.374 \\ 
Fraction of households of bad quality & 0.024 & 0.048 & 0.000 & 0.008 & 0.889 \\ 
% Fraction in Conventillo & 0.015 & 0.038 & 0.000 & 0.003 & 0.889 \\ 
HighSEG & 0.111 & 0.248 & 0.000 & 0.000 & 1.000 \\ 
MidSEG & 0.402 & 0.327 & 0.000 & 0.337 & 1.000 \\ 
LowSEG & 0.482 & 0.374 & 0.000 & 0.493 & 1.000 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
% \end{table} 



==> figs_tabs/summary_reg.tex <==
\begin{table}[!htbp] \centering 
%   \caption{} 
%   \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex]
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
$MobOut$ & 411 & 0.529 & 0.064 & 0.326 & 0.508 & 0.572 & 0.721 \\ 
$MobRisk$ & 411 & 0.893 & 0.444 & 0.240 & 0.648 & 1.004 & 5.381 \\ 
% $FracLock$ & 411 & 0.164 & 0.330 & 0 & 0 & 0 & 1 \\
% $R$ & 411 & 1.297 & 0.678 & 0.559 & 0.822 & 1.549 & 4.000 \\ 
\hline \\[-1.8ex] 
\end{tabular}
\caption{Summary statistics}
\label{tab:summ_stats}
\end{table} 
